I've Got 99 Problems But FLOPS Ain't One

Hyperscalers dominate the landscape of large network deployments, yet they rarely share data or insights about the challenges they face. In light of this supremacy, what problems can we find to solve in this space? We take an unconventional approach to find relevant research directions, starting from public plans to build a $100 billion datacenter for machine learning applications. Leveraging the language models scaling laws, we discover what workloads such a datacenter might carry and explore the challenges one may encounter in doing so, with a focus on networking research. We conclude that building the datacenter and training such models is technically possible, but this requires novel wide-area transports for inter-DC communication, a multipath transport and novel datacenter topologies for intra-datacenter communication, high speed scale-up networks and transports, outlining a rich research agenda for the networking community.

==> 3-2-cooling.tex <==
\subsection{Cooling}%
\label{sect:cooling}

In a May 2023 report, Microsoft argued for a datacenter that does not use water for
cooling. Further, more municipalities will require minimal, near-zero direct water
consumptions; otherwise, no building permits. \todo{Radu add source}

\textbf{Idea 1: Heat energy reuse.} The heat generated by datacenters can be
redirected to residential areas to help with household heating.
The Energy Reuse Factor (ERF) represents the fraction of total energy provided
that is actually employed for a secondary purpose.
In winter time, the potential ERF is 0.69, while in summer it rises to 0.86.

% Microsoft only provides numbers for datacenters of capacity 10MW and 40MW; 
% if we assume that the annual consumption is estimated using a linear function
% EAC(capacity) = m * capacity + b
%
% Then we have: m = (EAC(40) - EAC(10)) / (40 - 10) = 10533.33 MW
% b = EAC(40) - m*40 = -333.33 MW
%
% m*5GW + b = 52666333.33 MW = ~52.66 TW

Based on Microsoft's reported
numbers~\footnote{\url{https://local.microsoft.com/wp-content/uploads/2022/06/Azure_HeatReUse_Infographic.pdf}}
for datacenters of 10MW and 40MW, we can extrapolate that a 5GW datacenter would
have an ``estimated annual energy consumption'' of around 52.66 TW.
Employing the ERFs mentioned above and the cited figure of 6300KWh to heat a
household, this yields a potential 5.8 million households heated in winter,
which is more than the number of households in any American city.

\textbf{Idea 2: Water cooling.} Microsoft has made a pledge to become
``water-positive'' by the year 2030.
This term is vaguely defined, but generally implies that the amount of water
used for humidification, cooling etc. should be offset, possibly at some other
location, by water treatment or transportation.
So water cooling for a particular datacenter seems to still be on the table,
even with this target.

\emph{Adiabatic cooling.} Based on a Microsoft cooling methods
pamphplet~\footnote{\url{https://datacenters.microsoft.com/wp-content/uploads/2023/05/Azure_Modern-Datacenter-Cooling_Infographic.pdf}},
most of the USA is suitable for ``adiabatic cooling'', with Alaska being inside
the ``free air cooling'' zone.

% Microsoft provides the figures: 0.02 to 0.7 L/kWh:
% 0.02*5000000 = 100000
% 0.7*5000000 = 3500000
Adiabatic cooling comes in two forms: indirect evaporative cooling and direct
evaporative cooling.
For a 5GWh datacenter, the latter would consume between 100000 and 3500000
L/h of water.
% between 100 and 3500 cubic meters of water per hour



\emph{Free air cooling.} Free air cooling consumes no water for the cooling
process itself, though water may be used in winter for controlling humidity
levels.

% CyrusOne NVA9 - Sterling seems to require exclusively air chillers, with a
% surface of 65032 m^2 and a power consumption of 135 MW.
Current datacenters can dissipate at least 2.076 $kW/m^2$, which would require a
the 5GW datacenter to have a surface of ~2.41B $m^2$, slightly smaller than the
area of Luxembourg.

\emph{Immersion cooling.}

TODO


==> 6-related.tex <==
\section{Related Work}


==> 7-discussion.tex <==
\section{Discussion and Future Work}

\subsection{Inference}

While we've shown that training is possible at this scale, employing various
architectural choices, we've not yet talked about inference using the 2 models,
since our focus was primarily on the networking stack used during training.

For the Transformer model itself, the computation is similar to the pre-training
phase, except there is no more data parallelism (since there is no backward
pass). The tensor parallelism and pipeline parallelism stages are still needed,
but most of the communication time from the backward pass is now gone, so it no
longer becomes a networking issue.

We give our calculations of inference times, using the same formula from (ref
deepmind), calculated using different context sizes (tokens produced by the
model). We make the assumption that a full rack is holding one layer, so there's
a total of 224 racks needed for inference for the 100T model (while this doesn't
seem like it's fully utilizing the memory available, we discuss how to fill this
memory in the following paragraphs).

\todo[tabel]
Inference (ideal times, no PP, no TP):
100T
(512 tokens): 18 seconds (28.4 tokens per second)
(1024 tokens): 72 seconds (14.2 tokens per second)
(2048 tokens): 289 seconds (7.1 tokens per second)
(16000 tokens): 18664 seconds (0.85 tokens per second)
(32000 tokens): 71838 seconds (0.44 tokens per second)

50T
(512 tokens): 9.58 seconds (53 tokens per second)
(1024 tokens): 38 seconds (26 tokens per second)
(2048 tokens): 153 seconds (13.3 tokens per second)
(16000 tokens): 9504 seconds (1.68 tokens per second)
(32000 tokens): 38526 seconds (0.83 tokens per second)

We also note that there are multiple approaches to improve inference time. These
are, in no particular order:
- quantization: We already have a master model in FP8 weights, however we can
further reduce the weights precision level, to improve performance
- using a smaller, predictive model: there's a line of research (ref) that tries
to use much smaller models to predict tokens that are trivial to infer (e.g.
there are words that occur with very high frequency after other words,
especially interjections, particles, etc., and can be easily predicted by a
smaller model in size); the 100T / 50T model would be fed multiple tokens at
once from the small models, instead of being fed only 1 new token at a time, the
one that it itself predicted; this can dramatically improve inference time
- distillation: this line of research, similarly to quantization, looks at
compressing the knowledge of the model using smaller (or less) weights. In
particular, distillation tries to train a smaller model (a student network) from
a bigger model (a teacher network); the advantage of training the small model
from scratch is that the bigger model can give the smaller model much higher
throughput / signal of data, than if the small model would've learned from text
data itself (the big model can give the small model vectors in hidden dimension,
instead of text tokens).
- smart dynamic batching (using different batch size, scaling with load): this
approach looks at smartly batching incoming user requests, and adjusts a batch
size dynamically (i.e. more load, bigger batch size -> this translates into
slower inference per batch, but much better in total compared to doing single
batch inference; less load -> more compute "wasted" overall, but faster response
times); this method can fill the empty memory of GPUs

\subsection{Fault tolerance}


==> space-tricks.tex <==
%space left between floats.
%\setlength{\floatsep}{4mm}
% space between last top float or first bottom float and the text.
%\setlength{\textfloatsep}{2mm}

% space left on top and bottom of an in-text float.
\setlength{\intextsep}{0.5mm}
% space above caption
\setlength{\abovecaptionskip}{2mm}
%space below caption
\setlength{\belowcaptionskip}{0mm}

%% Change figure handling
%\renewcommand{\topfraction}{0.9}
%\renewcommand{\textfraction}{0.1}
%\renewcommand{\floatpagefraction}{1}

%\usepackage[small,compact,noindentafter]{titlesec} 
\usepackage[compact]{titlesec}

\titlespacing\section{0pt}{6pt plus 2pt minus 2pt}{2pt plus 2pt minus 2pt}
\titlespacing\subsection{0pt}{4pt plus 2pt minus 2pt}{2pt plus 1pt minus 1pt}
\titlespacing{\paragraph}{0pt}{2pt plus 0pt minus 1pt}{1.0ex}

%\usepackage[inline]{enumitem}
%\setlist{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}

\usepackage[subtle,lists,paragraphs]{savetrees}
% \usepackage[moderate]{savetrees}

\usepackage{setspace}
\usepackage[margin=0pt,skip=0pt,font={stretch=0.9}]{caption}
%\usepackage[margin=5pt,font={stretch=0.9}]{caption}
%\usepackage[margin=8pt,font={small,bf,stretch=0.85}]{caption}

%\titleformat{\subsection}
%  {\normalfont\fontsize{12}{15}\bfseries}{\thesection}{1em}{}

